Isomorphisms of Class S Theories with IndexLab

We use IndexLab to scan untwisted and twisted class $\mathcal{S}$ constructions based on ADE Lie algebras of rank up to seven, as well as $A_8$ and $E_8$. We consider surfaces of genus at most three with up to five punctures, covering 167,244,647 constructions in total. To find candidate pairs of isomorphic theories, we compare Schur and Hall-Littlewood indices, Weyl anomalies, Coulomb branch spectra, and flavor data. We set aside pairs explained by known mechanisms, leaving a catalogue of 5,278 candidate pairs. Recurring changes in rank, puncture labels, and twists suggest families of candidate isomorphisms. We group 99.58% of the pairs into 25 families and 6 finite families. IndexLab is available at superconformal.com.

==> figures/Family_Diagrams_Orbits.tex <==
% Draw a Bala--Carter label and its weighted Dynkin diagram.
% The digit string follows the node order in IndexLab's HLData.
\makeatletter
\newcount\AtlasOrbitNodeIndex

\newcommand{\AtlasOrbitNode}[3]{%
  \put(\number\numexpr#1-4\relax,\number\numexpr#2-4\relax){%
    \framebox(8,8){$\scriptstyle #3$}%
  }%
}

\newcommand{\AtlasOrbitEGraph}[2]{%
  \edef\AtlasOrbitStart{\number\numexpr49-6*(#1-2)\relax}%
  \edef\AtlasOrbitEdges{\number\numexpr#1-2\relax}%
  \edef\AtlasOrbitBranch{\number\numexpr\AtlasOrbitStart+24\relax}%
  \multiput(\number\numexpr\AtlasOrbitStart+4\relax,8)(12,0){\AtlasOrbitEdges}{\line(1,0){4}}%
  \put(\AtlasOrbitBranch,12){\line(0,1){2}}%
  \AtlasOrbitNodeIndex=0
  \@tfor\AtlasOrbitWeight:=#2\do{%
    \advance\AtlasOrbitNodeIndex by 1
    \ifnum\AtlasOrbitNodeIndex=#1\relax
      \AtlasOrbitNode{\AtlasOrbitBranch}{18}{\AtlasOrbitWeight}%
    \else
      \AtlasOrbitNode{\number\numexpr\AtlasOrbitStart+12*(\AtlasOrbitNodeIndex-1)\relax}{8}{\AtlasOrbitWeight}%
    \fi
  }%
}

\newcommand{\AtlasOrbitFGraph}[1]{%
  \put(35,8){\line(1,0){4}}%
  \multiput(47,7.3)(0,1.4){2}{\line(1,0){4}}%
  \put(59,8){\line(1,0){4}}%
  \qbezier(48.5,6)(49.7,7)(50.9,8)%
  \qbezier(48.5,10)(49.7,9)(50.9,8)%
  \AtlasOrbitNodeIndex=0
  \@tfor\AtlasOrbitWeight:=#1\do{%
    \AtlasOrbitNode{\number\numexpr31+12*\AtlasOrbitNodeIndex\relax}{8}{\AtlasOrbitWeight}%
    \advance\AtlasOrbitNodeIndex by 1
  }%
}

\newcommand{\AtlasOrbitGGraph}[1]{%
  \multiput(47,6.6)(0,1.4){3}{\line(1,0){4}}%
  \qbezier(49.5,6)(48.3,7)(47.1,8)%
  \qbezier(49.5,10)(48.3,9)(47.1,8)%
  \AtlasOrbitNodeIndex=0
  \@tfor\AtlasOrbitWeight:=#1\do{%
    \AtlasOrbitNode{\number\numexpr43+12*\AtlasOrbitNodeIndex\relax}{8}{\AtlasOrbitWeight}%
    \advance\AtlasOrbitNodeIndex by 1
  }%
}

\newcommand{\AtlasOrbit}[3]{%
  \begingroup
  \setlength{\unitlength}{1pt}%
  \linethickness{0.32pt}%
  \edef\AtlasOrbitSeries{\@car#2\@nil}%
  \edef\AtlasOrbitRank{\@cdr#2\@nil}%
  \def\AtlasOrbitE{E}\def\AtlasOrbitF{F}%
  \begin{picture}(98,30)
    \put(49,26){\makebox(0,0){\footnotesize\ensuremath{#1}}}%
    \ifx\AtlasOrbitSeries\AtlasOrbitE
      \AtlasOrbitEGraph{\AtlasOrbitRank}{#3}%
    \else\ifx\AtlasOrbitSeries\AtlasOrbitF
      \AtlasOrbitFGraph{#3}%
    \else
      \AtlasOrbitGGraph{#3}%
    \fi\fi
  \end{picture}%
  \endgroup
}
\makeatother

